On the analyticity of the trajectories of the particles in the patch problem for $2$D Euler and aggregation equations

We give a proof of the analiticity in time for the particle trajectories associated with the solutions of some transport equations when the initial datum is a patch. These results are obtained from a precise study of the Beurling transform, which provides estimates for the solutions of some new equations satisfied by the lagrangian flow.

==> Apxthm1.tex <==
% !TeX encoding = UTF-8
% !TeX spellcheck = ca_ES
% !TeX root = Analit4.tex 


\subsection{Equivalence of flows}


Let $\psi$ be the unique flow corresponding to the solution of the equation (E) or (A) with the initial condition $\varpi_0(z)$ or $\rho_0(z)$. 

Then, since both are transport equations, $\psi$ satisfies (7) in the case of Euler and (8) in the case of the aggregation, both depending only on an initial datum that we will call $\varpi_0$.

Let $\phi$ the analytic solution obtained in theorem 1 wiht the respective conditions. Observe that $a$ in this theorem is already determined. 

Let us assume that $\phi$ is also a flow. Then we can conclude that 

\begin{equation}\label{infty} \phi(z,\, t)=\psi(z,\, t)\ \  &\text{for}\ \  (z,\, t)\in\C\times[-T_0,\, T_0].\end{equation}



Both $\psi$ and $\phi$ generate vector fields $v$ and $u$, namely
$$v(\zeta,\, t)=\frac{\partial\psi}{\partial t}(\psi(\ ,\, t)^{-1}(\zeta),\, t)$$ and  
 $$u(\zeta,\, t)=\frac{\partial\phi}{\partial t}(\phi(\ ,\, t)^{-1}(\zeta),\, t).$$
 
 Since both $\psi$ and $\phi$ are solutions of the problems (7) or (8), we have that 
$$\frac{\partial v}{\partial\zeta}(\zeta,\, t)=\varpi(\zeta,\, t)=\varpi_0(\psi(\ ,\, t)^{-1}(\zeta),\, t)$$ and  $$\frac{\partial u}{\partial\zeta}(\zeta,\, t)=\varpi(\zeta,\, t)=\varpi_0(\phi(\ ,\, t)^{-1}(\zeta),\, t)$$  in $\C\setminus\partial\Omega$.

 (trajectories).

Then $$\frac{\partial (u-v)}{\partial\zeta}(\zeta,\, t)=0$$ for $\zeta$ outside a subset of $\C$ of $0$ analytic capacity. since $u$ and $v$ are bounded and vanish at infinity., by Liouville's theorem we conclude that $u\equiv v$. This conclude.
 
 
 \newpage

\subsection{Size properties} 

We have seen that $$\phi(z,\, t)=z+\sum_{s=1}^\infty \xi^{(s)}(z)\, t^s\stackrel{def}{=}z+A(z,\, t)$$ and $$\xi^{(s)}(z)=\bar C[\theta^{(s)}](z)$$

\begin{lem} There exists  $T_0>0$ and $K>0$ such that for $|t|\le T_0$, we have $$\|A(\ ,\, t)\|_{L^\infty(\C)}\le K$$ and $$\|\nabla_zA(\ ,\, t)\|_{L^\infty(\C)}<\le\frac{1}{2}.$$
	
	\end{lem}
\begin{proof} Since $$\sum_{s=1}^N\|\xi^{(s)}\|_{L^\infty(\C)}\, \tau^s=\sum_{s=1}^N\|\bar C[\theta^{(s)}]\, \|_{L^\infty(\C)}\, \tau^s$$ and $$\|\bar C[\theta^{(s)}]\, \|_{L^\infty(\C)}\, \le C\{\|\theta^{(s)}\, \|_{L^\infty(\C)}+\|\theta^{(s)}\, \|_{L^p(\C)}\}$$ wiht $C$ independent of $s$ and $N$, and $1<p<2$, due to the Lemmma ($\||\ \||$), we obtain the first inequality.
	
	\bigskip
	
	On the other hand $$\sum_{s=1}^N\|\nabla_z\xi^{(s)}\|_{L^\infty(\C)}\, \tau^s\le\sum_{s=1}^N\{\|\theta^{(s)}\|_{L^\infty(\C)}+\|\bar B[\theta^{(s)}]\|_{L^\infty(\C)}\}\, \tau^s$$
	$$\le K\, \sum_{s=1}^N\|\theta^{(s)}\|_{\gamma}\, \tau^s$$ where $K$ is independent of $s$ and $N$. We have used the part of theorem 3.
	\end{proof}
\bigskip
\bigskip

\subsubsection{$\phi$ is a flow.}

\begin{prop} \begin{enumerate}
		\item $\phi(\C,\, t)$ is closed for every $t$.
		
		\bigskip
		
		\item $\phi(\ ,\, t)$ is one to one. 
		
			\bigskip
		
		\item $\phi(\C ,\, t)$ is open. 
		
			\bigskip
		
		\item $\phi(\ ,\, t)$ is an homeomorphism and differentiable in $\C\setminus\partial\Omega$. 
	\end{enumerate}
	
	\end{prop}

\begin{proof} \begin{enumerate}
		\item If $w_l=\phi(z_l,\, t)=z_l+A(z_l,\, t)$ is a sequence such that $w_l\rightarrow w_0$, then $|z_l|\le |w_l|+|A(z_l,\, t)|\le M+\|A(\ ,\, t)\|_{L^\infty},$ where $M$ is a bound for $w_l$. Then there exists a partial sequence $z_{l_s}\rightarrow z_0$
		and since $\phi(\ ,\, t)$ is a continuous map then $w_0=\phi(z_0,\, t)$.
		
		
		\bigskip
		
		\item Since $$\phi(z,\, t)-\phi(z',\, t)=z-z'+A(z,\, t)-A(z',\, t),$$ and $\nabla A(\ ,\, t)$ exists almost everywhere in $\C$ and $\|\nabla A(\ ,\, t)\|_{L^\infty}<1$ if $|t|\le T'''_0$, then by Rademacher's theorem $A(\ ,\, t)\in Lip(1,\, \C)$, so if $\phi(z,\, t)-\phi(z',\, t)=0$, then $|z-z'|<|z-z'|$. That's a contradiction. 
		
		\bigskip
		
		\item Since for some $\tilde T\in(0,\, T'''_0]$ we have $|J_zA(z,\, t)|<\frac{1}{2}$ for $(z,\, t)\in(\C\setminus\partial\Omega)\times[-\tilde T,\, \tilde T]$, and $\phi(\ ,\, t)\in\ka{\infty}(\C\setminus\partial\Omega)$, then  $\phi(\C\setminus\partial\Omega ,\, t)$ is open and $\phi(\ ,\, t)$ is a diffeomorphism on the image, because of the e inverse function theorem and theinjectivity.
		
		\medskip 
		
		The injectivity of $\phi(\ ,\, t)$ also implies that $$\phi(\partial\Omega,\, t)=\partial\phi(\Omega,\, t)\cap\partial\phi(\bar\Omega^c,\, t):$$
		
		Since for $w_0=\phi(z_0,\, t)$, with $z_0\in\partial\Omega$, we have that $z_0=\lim z_l=\lim z'_l$ where $z_l\in\Omega$ and $z'_l\in\bar\Omega^c$, then $w_0=\lim\phi(z_l,\, t)=\lim\phi(z'_l,\, t)$. This implies $\subset$.
		
		On the other hand, for $w_0\in\partial\phi(\Omega,\, t)\cap\partial\phi(\Omega^c,\, t)$ we have that $w_0=\lim\phi(z_l,\, t)=\lim\phi(z'_l,\, t)$, where $z_l\in\Omega$ and $z'_l\in\bar\Omega^c$, so $z_l=w_0-A(z_l,\, t)$ and $z'_l=w_0-A(z'_l,\, t)$ and there are partial subsequences $z_{l_j}\to\alpha\in\bar\Omega$ and $z'_{l_k}\to\beta\in\Omega^c$. Then $\phi(\alpha,\, t)=\phi(\beta,\, t)=w_0$. The injectivity of $\phi(\ ,\, t)$ implies $\alpha=\beta\in\partial\Omega$. 
		
		\medskip
		
		In fact, $\phi(\ ,\, t)$ transforms boundaries in boundaries:
		
		$$\phi(\partial\Omega ,\, t)=\partial\phi(\Omega,\, t)=\partial\phi(\bar\Omega^c ,\, t),$$ because $\phi(\partial\Omega ,\, t)\subset\partial\phi(\Omega,\, t)$ by continuity, and if $w_0\in\partial\phi(\Omega,\, t)\subset\overline{\phi(\C,\, t)}=
		\phi(\C,\, t)$, then $w_0=\phi(z_0,\, t)$ for a unique $z_0\in\C$. 
		
		We have that $z_0\notin\Omega$ because then $w_0\in\phi(\Omega,\, t),$ an open set, and similarely $z_0\notin\bar\Omega^c$. So $z_0\in\partial\Omega$.
		
		The same argument can be performed for $\partial\phi(\bar\Omega^c,\, t)$.
		
		\medskip
		
		And, as $\Omega$ is a bounded subset of $\C$, we finally conclude that $$\partial\phi(\bar\Omega,\, t)=\phi(\partial\Omega,\, t),$$ because if $w\in\partial\phi(\bar\Omega,\, t),$ then $w\in\phi(\bar\Omega,\, t),$ so $w=\phi(z,\, t),$ for $z\in\bar\Omega$, and in fact $z\in\partial\Omega$ because $\phi(\Omega,\, t)$ is open. Also if $w\in\phi(\partial\Omega,\, t),$ then $w=\phi(z,\, t),$ for $z\in\partial\Omega$. Then $z=\lim z_l$ for $z\in\Omega$, so $w\in\partial\phi(\bar\Omega,\, t),$ and also $z=\lim \zeta_l$ for $\zeta\in\bar\Omega^c\subset\Omega^c$, so $w\in\phi(\bar\Omega,\, t)^c.$ All this implies that $w\in\partial\phi(\Omega,\, t),$ 
		
		\medskip
		
		As a consequence of all these facts, $$\phi(\C,\, t)=\C$$.
		
		If $w_0\in\C\setminus\phi(\C,\, t)$, let $w_1=\phi(z_1,\, t)$ a point satisfiying $|w_0-w_1|=d(w_0,\, \phi(\C,\, t))$. Clearly $z_1\in\partial\Omega$ because $\phi(\Omega,\, t)$ and $\phi(\bar\Omega^c,\, t)$ are open sets. In fact, $$w_1\in\partial\phi(\Omega,\, t)\cap\partial\phi(\bar\Omega^c,\, t)\cap\partial\phi(\C,\, t).$$
		
		On the other hand, $\phi(\partial\Omega,\, t)$ is a Jordan curve in $\C$, and then it divides $\C$ in two disjoint regions, say $\Pi_+$ and $\Pi_-$ and the curve itself: $$\C=\Pi_+\cup\phi(\partial\Omega,\, t)\cup\Pi_-,$$ and $\Pi_-$ is bounded.
		
		Let us prove now that $\phi(\Omega,\, t)\subset\Pi_-$. Since $\phi(\bar\Omega,\, t)$ is a compact set and then there is a large ball $B_R(0)$ such that $$\phi(\bar\Omega,\, t)\cup\Pi_-\subset\overline{B_R(0)}.$$ If $u_0\notin B_{2R}(0)$, then $u_0\in\Pi_+$ and if we assume that $\phi(\Omega,\, t)\subset\Pi_+$, then since $\Pi_+$ is arc-connected there must exist a continuous curve $$p:[0,1]\rightarrow\Pi_+$$ and a point $z_2\in\Omega$ such that $p(0)=u_0$, $p(1)=\phi(z_2,\, t)$. By connection arguments this implies that $p([0,\, 1])\cap\partial\phi(\bar\Omega,\, t)\neq\emptyset$, so $\partial\phi(\Omega,\, t)\setminus\phi(\partial\Omega,\, t)\neq\emptyset$. That's a contradiction. 
		
		\medskip
		
		Using the same arguments, we also prove that $\phi(\bar\Omega^c,\, t)\subset\Pi_+$. Let us show now that in fact $\phi(\Omega,\, t)=\Pi_-$ and $\phi(\bar\Omega^c,\, t)=\Pi_+$. If $w_0\in\Pi_+\setminus\phi(\bar\Omega^c,\, t)$ There exists an arc in $\Pi_+$, $p$,  joining $w_0$ with a point in $\phi(\bar\Omega^c,\, t)$. Again this arc must cross the curve $\phi(\partial\Omega^c,\, t)$. that's a contradiction.  
		
		\bigskip
		
		\item $\phi(\ ,\, t)$ is an homeomorphism and differentiable in $\C\setminus\partial\Omega$. 
	\end{enumerate}
	
	\end{proof}
\bigskip
\bigskip




\bigskip
\bigskip


\subsubsection{Boundedness of the velocity.}

Sionce $\phi$ is a flow, we can define 
$$\frac{\partial\phi}{\partial t}(\phi(\ ,\, t)^{-1}(\zeta),\, t)=u(\zeta,\, t).$$

We will prove that $u(\ ,\, t)\in(\ka{}\cap L^\infty)(\C)$ is bounded uniformely in $t$. This is equivalent to the same fact for $\frac{\partial\phi}{\partial t}(z,\, t)$ and $z\in\C$. 

Since $$\frac{\partial\phi}{\partial t}(z,\, t)=\frac{\partial A}{\partial t}(z,\, t)=\sum_{s=1}^\infty s\, \bar C[\theta^{(s)}](z)\, t^{s-1}$$ 


